ProBE: Proportioning Privacy Budget for Complex Exploratory Decision Support

This paper studies privacy in the context of complex decision support queries composed of multiple conditions on different aggregate statistics combined using disjunction and conjunction operators. Utility requirements for such queries necessitate the need for private mechanisms that guarantee a bound on the false negative and false positive errors. This paper formally defines complex decision support queries and their accuracy requirements, and provides algorithms that proportion the existing budget to optimally minimize privacy loss while supporting a bounded guarantee on the accuracy. Our experimental results on multiple real-life datasets show that our algorithms successfully maintain such utility guarantees, while also minimizing privacy loss.

==> entropyalgos.tex <==
\section{Multi-Step/Entropy-based/Predicate-wise DP Algorithms}
\subsection{MIDE Algorithms}
MIDE \cite{mide} proposed three algorithms which answer aggregate threshold queries under accuracy constraints:
Threshold-shift Laplace Mechanism (TSLM), the single step algorithm previously defined in Section 3, two multi-step algorithms, the Progressive Predicate-wise Laplace Mechanism (PPWLM), and its data-dependent version (DPPWLM).

PPWLM aims to improve on TSLM by progressively tightening the uncertain region $u$ around the threshold based on the aggregate values of each predicate in a set number of steps $m$. For a single aggregate threshold query, the algorithm starts with a small privacy budget $\epsilon_s$ and increases it in geometric increments every iteration. The final $\beta$ of this mechanism is divided equally across iterations $\beta/m$ and the privacy loss per iteration is bounded by the final privacy budget $\epsilon_m=\frac{\Delta g\ln(1/(2\beta/m))}{u}$.

DDPWLM builds upon the previous mechanism by dynamically updating the next iteration's privacy budget,
uncertain region and false negative rate in such a way that the privacy metric \textit{min-entropy} is at its highest. 
Instead of predetermining the privacy budget of each iteration, DDPWLM chooses the next iteration's $\epsilon$ by calculating the probabilities of each predicate being higher/lower than the shifted threshold using previous noisy aggregated values. These probabilities 
are used to calculate the min-entropy, and the highest value is used to choose the optimal privacy budget $\epsilon$. This algorithm similarly bounds the $\beta$ per iteration equally to $\beta/m$, therefore setting the worse-case privacy loss per iteration to be $\epsilon_m = \frac{\Delta g\ln(1/(2\beta/m))}{u}$.
\subsection{ProBE Optimizations}
% \begin{algorithm}[t] 
% \begin{algorithmic}[1]
% \Procedure{TslmProbe}{$Q, D, u, \beta,o,\Delta g,\epsilon_{max},t$}
% \State Let $O_f \gets \{\},\epsilon_f \gets 0$
% \For{$i=1,...,n$}
% \State $\beta_i \gets \frac{\Delta g_i \beta  \prod_{x=1}^{n,x\neq i } (u_x )}{o_i\sum_{y=1}^{n}\prod_{x=1}^{n,x\neq y } (u_x \Delta g_y )}$
% % \State $\beta_i \gets \frac{\beta  \prod_{x=1}^{n,x\neq i } (u_x )}{\sum_{y=1}^{n}\prod_{x=1}^{n,x\neq y } (u_x )}$  
% \State $O_i,\epsilon_i \gets$ \textsc{Tslm} ($Q_i,u_i,\beta_i,\epsilon_{max}$)
% \State $\epsilon_f \gets \epsilon_f + \epsilon_i$
% \If{$\epsilon_f \leq \epsilon_{max}$}
% \If{$t_i=0$}
% \State $O_f \gets O_i$ if $O_f = \emptyset$ else $O_f \gets O_f \cap O_i$
% \If{$O_i = \emptyset$} \Return $O_f,\epsilon_f$
% \EndIf
% \ElsIf{$t_i =1$}
%  \State $ O_f \gets O_f \cup O_i$
% \EndIf
% \Else
% \State \Return `Query Denied'
% \EndIf
% \EndFor
% \State \Return $O_f,\epsilon_f$
% \EndProcedure
% \end{algorithmic}
% \caption{ProBE-based Threshold Shift Laplace Mechanism. $Q=\{Q_1,...,Q_n\}$, $u=\{u_1,...,u_n\}$, $o= \{o_1,...,o_n\}$, $\Delta g=\{\Delta g_1,...,\Delta g_n\}$, $t=\{t_1,...,t_n\}$ where $t_i=0$ if conjunction, $1$ if disjunction}\label{algo:tslm}
% \end{algorithm}
We implement our ProBE optimization through two algorithms which use the existing mechanisms described in the previous section: the ProBE-based TSLM (Algorithm \ref{algo:tslm}), and the Probe-based Multi-Step Predicate-wise Laplace Mechanism (MSPWLM), which represents the class of iterative algorithms that includes both PPWLM and DDPWLM (Algorithm \ref{algo:ddpwlm}). %put note here
Both algorithms use our generalized apportionment technique as defined in Eq. \eqref{eq:gen_beta_occ} to determine the $\beta_i$ budget used by the existing algorithms on each atomic query to return individual privacy losses $\epsilon_i$. 
Note that because the apportionment equations for $\beta$ and $\gamma$ bounds are identical, we can pass our $\gamma_i$ values into the $\beta_i$ variables for both algorithms to evaluate our approach in the case of combined conjunction/disjunction and correlated sub-queries. For the multi-step algorithms, the apportionment is introduced by optimizing the final privacy budget for each sub-query $\epsilon_m$, meaning the worst case privacy loss will still be minimized while satisfying the false negative rate guarantee. This is done by setting the original $\beta_i$ budget for each atomic query to Eq. \eqref{eq:gen_beta_occ} divided equally across $m$ iterations. The overall privacy loss is thus progressively computed as the sum of $\epsilon_1,...\epsilon_n$, and
the resulting sets $O_i$ are either unioned or intersected depending on whether the query is a conjunction or a disjunction. 

We now present implementation optimizations introduced to further improve existing mechanisms in terms of privacy loss.
% This mechanism (Algorithm \ref{algo:tslm}) directly implements the algorithm discussed in the previous section. It compares each noisy aggregate for $Q_i$
% with a shifted threshold $c_i-u_i$, where each false negative bound $\beta_i$ is defined according to the equation in Eq. \eqref{eq:gen_beta_occ}. The set $O_i$ consists the predicates that have noisy aggregates greater than the shifted thresholds for $Q_j$, i.e. $g_j(D_{\lambda_{i}})+\eta_i > c_{i,j} -u_j$. The algorithm returns the union of $O_i$ for a disjunction query (line 13), or the intersection of $O_i$ for a conjunction query (line 9).

\noindent\textbf{Early stopping for conjunction queries.} For the conjunction of $n$ aggregate threshold queries, we note that the result of running a privacy-preserving mechanism like $M(D)=M_1(D)\cap M_2(D) ...$ $\cap \ M_n(D)$ on such a query can be determined as false if one sub-mechanism $M_i(D)$ is evaluated as false due to the nature of the intersection operator. We exploit this fact by adding an early stopping optimization which immediately exits if any of the sub-mechanisms return an empty set, thus bypassing the need to evaluate subsequent sub-mechanisms and further minimizing overall privacy loss and false negative rate. We include this optimization in Algorithm 1 (lines 10-11) and Algorithm 2 (lines 13-15), which exits the overall algorithm if the current sub-query's result set $O_i$ is empty and returns the current privacy loss $\epsilon_f$ and result set $O_f$.
\begin{theorem}
Algorithm 1 satisfies $\epsilon_{\max}$-DP and a $\beta$-bound FNR. If none of the atomic queries $Q_i$ are denied, the overall query's ex-post DP cost is $\epsilon \leq \sum_{i=1}^n \frac{\Delta g_i\ln(1/(2\beta_i)}{u_i}$.
\label{def:tslm}
\end{theorem}
% \subsection{PRoBE-based Multi-Step Mechanisms}
% \textcolor{red}{We implement our ProBE optimization through two multi-step algorithms defined in previous work \cite{mide}, the Progressive Predicate-wise Laplace mechanism (PPWLM), and the Data-Dependent Predicate-wise Laplace mechanism (DDPWLM).}
 % We now adapt these algorithms to answer complex decision queries composed of multiple conjunctions and/or disjunctions. We group both PPWLM and DDPWLM into a class of mechanisms entitled Multi-Step Predicate-Wise Laplace Mechanism (MSPWLM), which will be called in our ProBE-based iterative mechanism. We choose to run MSPWLM for each sub-query in a fixed number of steps $m$ across all sub-queries, and optionally, a fixed fine-grained steps $m_f$. We introduce our ProBE solution by optimizing the final privacy budget for each sub-query, meaning the worst case value for $\epsilon$ will still be minimized while satisfying the false negative rate guarantee. This is implemented by setting the false negative rate of each sub-query $\beta_i$ to the expression in Eq. (\ref{eq:gen_beta_occ}), and subsequently dividing it equally across $m$-steps (line 8). The algorithm then calls the original MSPWLM algorithm using the $\beta_i$ defined for each sub-query (line 9). We further modify both original PPWLM and DDPWLM algorithms to implement $\beta$ budget tracking: during each sub-query execution, we keep track of and return the remaining $\beta_i$ budget which was not spent by the current sub-query.
 % If the current overall privacy cost is lower than the maximum privacy budget allowed, the resulting set is either unioned or intersected with the previous results depending on whether the query is a conjunction or a disjunction (lines 12-18). We additionally implement the early stopping technique for conjunction (lines 13-15) that exits the algorithm if the current sub-query does not return any elements (i.e. the $O_i$ set is empty), thus potentially saving on privacy loss for such queries.
\noindent
\textbf{$\beta$-Budget Redistribution}. In the case of multi-step algorithms, we exploit their iterative nature to further optimize $\beta$ budget allocation during execution. Given that certain queries may terminate early (if an iteration $j<m$ yields no predicates within the uncertain region), the assigned $\beta_i$ for such a query may not be fully used and may thus be wasted. We exploit the progressive nature of such algorithms to further optimize the privacy budget: if the previous sub-query terminates before the $m$-th step of its run, we can redistribute the leftover false negative rate budget to subsequent sub-queries, thus fully utilizing the false negative rate bound given and consequently minimizing the overall privacy loss. For each sub-query, we calculate the remaining $\beta$ budget after running the MSPWLM algorithm by subtracting the used $\beta_i$ budget from the overall $\beta$  (line 10). For subsequent sub-queries, we check if the remaining $\beta$ budget $\beta_{rem}$ from the previous iteration is higher than 0. If this is not the case, then we use the ProBE optimization with the original $\beta$ and all the sub-queries. Otherwise, we update the overall $\beta$ to the remaining $\beta_{rem}$ and re-run the ProBE optimization using only the subsequent sub-queries $Q_i, \ldots ,Q_n$ and their corresponding uncertain regions (lines 4-6). To illustrate this algorithm, we use the example below.
% \vspace{-5mm}
\begin{algorithm}[t] 
\begin{algorithmic}[1]
\Procedure{MSpwlmProbe}{$Q, D, u, \beta,o,\Delta g, \epsilon_{max},\epsilon_s,m,m_f,t$}
\State Let $O_f \gets \{\},\epsilon_f \gets 0,\beta_{rem} \gets 0$
\For{$i=1,...,n$}
\If{$\beta_{rem} > 0 $}
\State update overall FNR budget $\beta \gets \beta_{rem}$
\State $Q \gets \{Q_{i},...,Q_n\}$ and $u = \{u_i,...,u_n\}$
\EndIf
\State $\beta_i \gets \frac{\Delta g_i \beta  \prod_{x=1}^{n,x\neq i } (u_x )}{o_i\sum_{y=1}^{n}\prod_{x=1}^{n,x\neq y } (u_x \Delta g_y )}$
\State $O_i, \epsilon_{i}, \beta_{used} \gets$ \textsc{Mspwlm}($Q_i,u_i,\beta_i,\epsilon_{max},\epsilon_{s_i},m,m_f$)
\State $\beta_{rem} \gets 0$ if $\beta_i=\beta_{used}$ else $\beta - \beta_{used}$ 
\State $\epsilon_f \gets \epsilon_f + \epsilon_i$
\If{$\epsilon_f \leq \epsilon_{max}$}
\If{$type = 0$}
\State $O_f \gets O_{i}$ if $O_f = \emptyset$ else $O_f \gets O_f \cap O_{i}$
\State \Return $O_f,\epsilon_f$ if $O_{i} = \emptyset$

\ElsIf{$type =1$}
\State $ O_f \gets O_f \cup O_{i}$
\EndIf
\Else
\State \Return `Query Denied'
\EndIf
\State \Return $O_f,\epsilon_f$

\EndFor
\EndProcedure
\end{algorithmic}
\caption{ProBE-based Multi-Step Predicate Wise Laplace Mechanism. $Q=\{Q_1,...,Q_n\}$, $u=\{u_1,...,u_n\}$, $\epsilon_s = \{\epsilon_{s_1},...,\epsilon_{s_n}\}$, $o= \{o_1,...,o_n\}$, $\Delta g=\{\Delta g_1,...,\Delta g_n\}$, $t=\{t_1,...,t_n\}$  where $t_i=0$ if conjunction, $1$ if disjunction}\label{algo:ddpwlm}
\end{algorithm}
\begin{exmp}Consider a 3-step PPWLM run with a conjunction query composed of 4 aggregate threshold queries; if the first query finishes executing after its 1st step, its leftover overall false negative rate will be $\beta - \Delta\beta_1$, where  $\Delta\beta_1=\frac{1}{3}\beta_1$. Therefore we re-compute the false negative rates for subsequent queries $\beta_2,\beta_3,\beta_4$ using Eq. (\ref{eq:gen_beta_occ}) with $\beta' = \beta - \Delta\beta_1$ and with the $Q_2,Q_3,Q_4$ leftover queries.
\end{exmp}
\begin{theorem}
Algorithm 2 satisfies $\epsilon_{\max}$-DP and a $\beta$-bound FNR. If none of atomic queries $Q_i$ are denied, the overall query's ex-post DP cost is $\epsilon \leq \sum_{i=1}^n \frac{\Delta g_i\ln(1/(2\beta_i/m))}{u_i}$.
\label{def:mspwlm}
\end{theorem}
% \vspace{-10mm}

% We introduce our ProBE optimization by again minimizing the final privacy budget per iteration for each sub-query. This is done by setting the false negative rate of each sub-query $\beta_i$ to Eq. (\ref{eq:{gen_beta}_occ}) divided by the number of iterations $m$ (line 8), and subsequently using this rate when calling the original DDPWLM algorithm on every sub-query (line 9). We additionally modify the original algorithm to keep track and return the amount of $\beta_i$ budget used per sub-query $\beta_{used}$, which we use to calculate the remaining overall false negative rate $\beta_{rem}$. Note that we keep track of this rate due to the fact that the false negative rate used in the data-dependent algorithm is not fixed like in the progressive algorithm, but rather changes based on the optimal privacy budget chosen per iteration which minimizes entropy. The budget redistribution algorithm is similarly implemented in the data-dependent algorithm; the remaining $\beta$ budget is checked every sub-query, and if this rate is higher than 0 then we recompute the ProBE-optimized $\beta_i$ budgets using the remaining overall false negative rate budget $\beta_{rem}$ on the leftover sub-queries $Q_i,...,Q_n$ and their corresponding uncertain regions (lines 4-6). The overall privacy budget is progressively computed by adding each ex-post DP cost $E_i$ resulting from individual sub-queries.



==> experiments.tex <==
\section{Experiments}
In this section, we evaluate the three algorithms previously explained (Algorithms \ref{algo:ssprobe}, \ref{algo:tsprobe} and \ref{algo:ddpwlm}) on different real-life datasets based on various decision support application types. We assess their performance using a varying number of complex queries, and provide examples of queries modeled after frequently used KPIs and show their resulting privacy and accuracy levels. Our experiments prove that all ProBE-based algorithms achieve their utility guarantees, while also successfully minimizing privacy loss for different levels of query complexity.
\subsection{Experimental Setup}
\textbf{Datasets}. To evaluate our approach, we use three real-world datasets from different domains. The first dataset, $\mathsf{NYCTaxi}$, is comprised of New York City yellow taxi trip records in 2020 \cite{nytaxi}, where the data consists of 17 attributes and approximately 3 million records. The second data set, $\mathsf{UCI Dataset}$, is comprised of occupancy data in 24 buildings at the University of California, Irvine campus collected from April to May 2019 \cite{tippers}. This data consists of 18 attributes and 5 million records. The final dataset, $\mathsf{TurkishMarketSales}$, stores records of sale transactions at a chain supermarket across Turkey in 2017 \cite{turkishsales}, where the data consists of 1.2 million records and 26 attributes.
% \vspace{-5pt}
\begin{table*}[!h]
% \resizebox{\textwidth}{!}{
\begin{tabular} { |c|c|c|c| }
\hline
{\bf Dataset} & {\bf Attributes used} & {\bf Predicates} & {\bf \# of predicates $p$} \\
\hline
UCI Dataset & *, age, userType, gender, groupName, office & room, date  & 41(rooms)*14(days)=574
 \\ 
\hline
Turkish Market Sales & *, region, netTotal, customerId, category, gender  & city, date &  43 (cities)*14(days)=602
\\ 
\hline
NYTaxi & *, fareAmnt, totalAmnt, paymentType, location, storeFwdFlag & location, date  & 34(location)*15(days)=476  \\
\hline
\end{tabular}
\caption{Datasets used for experiments and respective attributes/predicates used}
\label{tab:datasets}
\end{table*}
\begin{table*}[tb]
% \resizebox{\textwidth}{!}{
\begin{tabular} { |c|c|c| }
\hline
{\bf Sales KPI} & {\bf Definition} & {\bf Aggregate Functions}\\
\hline
Sales Volume & \# of sales & COUNT(*)
 \\ 
\hline
Regional Sales Volume & \# of sales in region & COUNT(*) where region=`A'
\\ 
\hline
User Retention Rate & \# of customers per period & COUNT(DISTINCT(customerId))
\\
\hline
Conversion Rate & \# of sales / \# of customers & COUNT(*), COUNT(DISTINCT(customerId))
\\ 
\hline
\end{tabular}
\caption{KPI-based Queries used for Sales Dataset experiments}
% \vspace{-10pt}
\label{tab:kpi}
\end{table*}

\noindent
\textbf{Query Benchmarks}. For each dataset, we model several meaningful aggregate threshold queries as summarized in Table \ref{tab:datasets}. In this paper, we present our experimental results for the COUNT aggregate function only. Queries with other aggregate functions (e.g. AVERAGE), which show similar results, are included in Appendix E.
As per our previous definition of conjunction/disjunction queries, all of our sub-queries have the same predicates but different filters on certain attributes (e.g. sub-queries on the UCI dataset all check the same 41 rooms every day for 14 days for the count of records with filters on different attributes). For the Sales dataset specifically, we model our queries based on frequently used retail and sales KPIs. Table \ref{tab:kpi} summarizes the KPIs used, their respective definitions, and the aggregate functions used to represent them. For example, to illustrate the User Retention Rate KPI, we evaluate the distinct count of customers that visited the specific business in a specific time period. For the UCI and NYTaxi datasets which do not have clearly defined KPIs, we select meaningful queries which are modeled based on anomaly detection or performance evaluation scenarios typically used in decision support applications, for example selecting statistics based on specific demographics (e.g. age, gender, etc.) or specific performance criteria  (e.g. fare amount is above the norm for a specific location). For each query, we select the corresponding threshold using the Z-score outlier detection method, to further emulate the concept of anomaly detection that decision support applications implement.

\noindent
\textbf{Parameters}
We evaluate our algorithms (ProBE-SS, ProBE-TS, ProBE-Ent), as well as the baseline method of evenly apportioning the $\gamma$ bound evenly across the sub-queries, which we refer to as the \textit{Naive} algorithm. For all algorithms, we set $\gamma = 0.0005$, a maximum privacy loss of $\epsilon_{max} = 5$, a starting uncertain region of  $u_0=20\%|D|$, ran over a 100 iterations. ProBE-Ent has $m=4$ maximum steps, and an additional $m_f=3$ of fine-grained steps.
\vspace{-2mm}
\subsection{Experimental Results}
\textbf{Privacy Results}. We use two privacy metrics to evaluate the performance of our ProBE optimization as implemented in the previously mentioned algorithms, ex-post differential privacy, denoted by $\epsilon$, and min-entropy, denoted by $\mathcal{H}_{min}(\Theta)$. We assess the ProBE-SS, ProBE-TS, ProBE-Ent algorithms on exclusive conjunction, exclusive disjunction, and a randomized combination of both for a varying number of sub-queries (1 to 6) in order to evaluate the effect of the operator on privacy loss and utility. For the purpose of this paper, we only include conjunction and the combination in Figure \ref{fig:privacyres}.

% \nl{we might need to remove the conjunction only results and move them to the appendix}

ProBE-Ent overall achieves the lowest or close to the lowest $\epsilon$ privacy loss across all datasets for conjunction, disjunction, and their combination. This is due to the fact that ProBE-Ent makes use of the underlying data distribution to progressively compute the results of the query at the lowest privacy cost, while also allowing for early stopping at a much lower privacy loss if all predicates are properly classified outside of the uncertain region. 
% The privacy loss for exclusive conjunction is noticeably lower than the exclusive disjunction, and tends to be almost constant for PPWLM and DDPWLM. This can be attributed to the early stopping algorithm implemented for conjunctions coupled with the early stopping implemented by both multi-step algorithms.
Note that the data-dependent algorithm does not always benefit from early stopping and might have a higher privacy loss than ProBE-TS, which largely depends on the distance of the data points from the thresholds. The second privacy metric, min-entropy, also shows that ProBE-Ent outperforms other algorithms and stays constant or suffers only from a small decrease as the number of sub-queries increases. This directly follows from the fact that ProBE-Ent is designed to maximize min-entropy at each iteration. We also note that ProBE-TS outperforms ProBE-Ent when the number of sub-queries are lower, which could be attributed to the benefit of maximizing min-entropy when the queries are more complex.

\begin{figure*}
\captionsetup[subfigure]{justification=centering}
    \centering
    \begin{subfigure}[b]{.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experiments/conjN/conjTAXI.png}
     \includegraphics[width=\textwidth]{figures/experiments/conjN/conjSALES.png}
     \includegraphics[width=\textwidth]{figures/experiments/conjN/conjUCI.png}
    % \caption{NYTaxi data Epsilon (top) and \\ Min-Entropy (bottom)}
    \end{subfigure}
\begin{subfigure}[b]{.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experiments/conjN/entropytaxiconj.png}
     \includegraphics[width=\textwidth]{figures/experiments/conjN/entropysalesconj.png}
     \includegraphics[width=\textwidth]{figures/experiments/conjN/entropyuciconj.png}
    % \caption{NYTaxi data Epsilon (top) and \\ Min-Entropy (bottom)}
    \end{subfigure}
    \begin{subfigure}[b]{.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experiments/comboN/comboTAXI.png}
     \includegraphics[width=\textwidth]{figures/experiments/comboN/comboSALES.png}
     \includegraphics[width=\textwidth]{figures/experiments/comboN/comboUCI.png}
    % \caption{NYTaxi data Epsilon (top) and \\ Min-Entropy (bottom)}
    \end{subfigure}
        \begin{subfigure}[b]{.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experiments/comboN/entropytaxicombo.png}
     \includegraphics[width=\textwidth]{figures/experiments/comboN/entropysalescombo.png}
     \includegraphics[width=\textwidth]{figures/experiments/comboN/entropyucicombo.png}
    % \caption{NYTaxi data Epsilon (top) and \\ Min-Entropy (bottom)}
    \end{subfigure}
    \caption{Privacy Loss in terms of Ex-Post DP $\epsilon$ and Min-Entropy $\mathcal{H}_{min}(\Theta)$ for 1-6 sub-queries at $\gamma=0.0005$ for Conjunction (columns 1-2) and Combined Conjunction/Disjunction (columns 3-4) using NYTaxi (row 1), Sales (row 2) and UCI (row 3) data. }
    \label{fig:privacyres}
\end{figure*}

\noindent
\textbf{Accuracy Results}. To evaluate our algorithms, we use two accuracy metrics, the FNR, which is defined as the number of false negatives $n_{fn}$ divided by the total number of positives $n_p$, and the FPR, defined as the number of false positives $n_{fp}$ divided by the total number of negatives $n_n$. These metrics are averaged over the number of iterations ran per algorithm, which we set to 100. We again use the default value of $\gamma=0.0005$. For the uncertain region parameter, we use a default $u_i = 12\%|D_i|$ for the single-step algorithm, and a larger value of $u_{i_0}$ for the multi-step algorithms. For the upper limit on false positives, we use a percentage of the number of predicates $p$ $fp_{max} =1\%p$.

All algorithms achieve the guaranteed bound of $\gamma=0.0005$ as seen in Figure \ref{fig:accuracyres}, where the FNR is zero as the number of sub-queries increases for all datasets (meaning that the FNP is 0 as well). For single-step algorithms (Naive, ProBE-SS), the FPR mostly sees a steady increase both in the conjunction-only and combination queries, whereas the multi-step algorithms (ProBE-TS, ProBE-Ent) successfully meet the bound on false positives $fp_{max}$ at a lower privacy loss due to the upper bound estimation and dynamic re-computation of the uncertain region parameter $u_{opt}$. The pattern, however, largely depends on the data distribution of the underlying dataset; e.g. for the Sales dataset we note that the FPR decreases as the number of sub-queries increases, which may be attributed to selectivity of the query along with the distance of the data points from their respective thresholds. 
% Similarly, the multi-step algorithms may have a higher FPR which increases with the number of sub-queries due to their lower privacy loss, as seen for example in Figure \ref{fig:combo}\subref{fig:combosales} with the Sales data PPWLM, but this is not always the case and depends on the data distribution of the underlying dataset. 
% For example, the resulting FPR for the UCI dataset (Figures \ref{fig:conj}\subref{fig:uciconj} and  \ref{fig:combo}\subref{fig:ucicombo}) is 0 for all algorithms regardless of the number of sub-queries, due to the distance of the data points from the threshold.

\noindent
\textbf{Query Trees and Operator Distribution}. As discussed in \secref{treestructure}, the structure of a query tree has an effect on the privacy loss. To evaluate the impact of operator distribution (i.e. distributing a conjunction over a disjunction and vice versa) we run our algorithms for the two queries illustrated in Figure \ref{fig:q-tree}: $Q_I = Q_1 \cup (Q_2 \cap Q_3)$ and $Q_{II} = (Q_1 \cup Q_2) \cap (Q_1 \cup Q_3)$. We run these queries on the Sales dataset with the default parameters of $\gamma = 0.0005$, as well as a starting uncertain region parameter of $u_0=20\%|D|$ and steps $m=4$, $m_f=3$ for ProBE-Ent. Figure \ref{fig:varyingdistrib} shows that the distributed query $Q_{II}$ incurs a higher ex-post privacy cost than the grouped query $Q_{I}$ for all four algorithms. Similarly, the FPR for single-step algorithms sees a slightly higher value for query $Q_{II}$ as compared to the original query $Q_{I}$. Experiments ran on distributing the AND operator over or (i.e. $Q_1 \cap (Q_2 \cup Q_3)$ vs. $(Q_1 \cap Q_2) \cup (Q_1 \cap Q_3)$) showed similar results.
\begin{figure*}
\captionsetup[subfigure]{justification=centering}
      \centering
    \begin{subfigure}[b]{.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experiments/conjN/conjAccTAXI.png}
  
    \label{fig:conjtaxi}
    \end{subfigure}
    \begin{subfigure}[b]{.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experiments/conjN/conjAccSALES.png}
   
    \label{fig:conjsales}
    \end{subfigure}
    \begin{subfigure}[b]{.32\textwidth}
    \label{fig:uciconj}
    \centering
    \includegraphics[width=\textwidth]{figures/experiments/conjN/conjAccUCI.png}

    \end{subfigure}
    \begin{subfigure}[b]{.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experiments/comboN/comboAccTAXI.png}
    \caption{NYTaxi data FNR (left axis) and FPR (right axis)}
    \label{fig:combotaxi}
    \end{subfigure}
    \begin{subfigure}[b]{.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experiments/comboN/comboAccSALES.png}
    \caption{Sales data FNR (left axis) and FPR (right axis)}
    \label{fig:combosales}
    \end{subfigure}
    \begin{subfigure}[b]{.32\textwidth}
    
    \centering
    \includegraphics[width=\textwidth]{figures/experiments/comboN/comboAccUCI.png}
   \caption{UCI  data FNR (left axis) and FPR (right axis)}
   \label{fig:ucicombo}
    \end{subfigure}
    \caption{ Accuracy in terms of False Negative Rate (FNR) and False Positive Rate (FPR) for 1-6 sub-queries at $\gamma=0.0005$ and $u=12\%$ for Conjunction-only (top row) and Combined Disjunction/Conjunction (bottom row).}
\label{fig:accuracyres}
\end{figure*}

% \nl{since we recompute the u in the two multi-step algos, we can change this experiment to vary the static u just for the single step algos, and vary the starting $u_0$ for multi-step algos.}
\noindent
\textbf{Varying Uncertain Region}. We vary the uncertain region $u$ to evaluate the performance of all four algorithms with values $u \in \{5,10,...,30\}$\% of the data range on the Sales dataset using the query $Q_1 \cup (Q_2 \cap Q_3)$. For the single-step algorithms, this is the $u$ parameter input by the user knowing the data distribution, whereas it corresponds to the multi-step algorithms' starting large uncertain region $u_0$ set internally. We fix the other parameters to $\gamma = 0.0005$, as well as $m=4$ and $m_f=3$ for ProBE-Ent. 
% \begin{table}[H]
%     \centering 
%     \begin{tabular}{|c|c|c|c|}
%     \hline
%     % \cline{2-4}
%     {\bf Correlation} & Negative& Low/None & Positive \\ \hline
%          {\bf FNR} & 0.0015 & 0.0 & 0.0  \\ \hline
%     \end{tabular}
%     \caption{False Negative Rate for Conjunction Query with Sub-Queries of Varying Correlation with $\gamma=0.0005$, $s_{min}=0.05$.}
%     \label{tab:corrQueries}
% \end{table}

Figure \ref{fig:varyingdistrib} shows that as the uncertain region increases, privacy loss declines for all algorithms as expected, seen in Figure \ref{fig:varyingdistrib}\subref{fig:varEp}. Whereas most algorithms see a steady decline in $\epsilon$, ProBE-Ent's privacy loss does not benefit from a higher $u$ starting around the value of $u=0.1$. This may attributed to the purpose of ProBE-Ent, which aims to minimize entropy rather than $\epsilon$, causing the algorithm to possibly run additional steps in order to achieve the highest Min-Entropy $\mathcal{H}_{min}(\Theta)$. We see that the privacy loss is not significantly different across algorithms, whereas the utility, specifically the FPR, sees the largest variance. For single-step algorithms, we see the FPR steadily increase as the uncertain region increases, which proves the direct correlation between false positives and $u$. However, the multi-step algorithms do not see this increase due to the enforced bound on false positives from the second step which recomputes the next optimal $u$. The FNR does not change due to the $\gamma$ bound guarantee.
% \nl{rerun exp}
% \noindent
% \textbf{Correlated Sub-Queries}. We evaluate how our approach performs when using the $\beta$-bound on FNR, and vary the correlation factor between sub-queries due to its direct effect on the $\beta$ bound as explained in \secref{independence} (i.e. our apportionment technique does not always guarantee a $\beta$-bound on FNR depending on the correlation factor between sub-queries). We compare three pairs of sub-queries on the Sales dataset with negative, low, and positive correlations using the Pearson correlation factor. We test each level on a 2-way conjunction query $Q = Q_1 \cap Q_2$ using the ProBE-SS algorithm with the default parameters of $\beta=0.0005$ and $u=12\%$. Table \ref{tab:corrQueries} shows that for all levels of correlation, we successfully achieve the $\gamma$-bound FNR. For negatively correlated sub-queries, the FNR is slightly higher, which is consistent with Eq. \eqref{eq:conjf}, but is still lower than $\gamma$.
\begin{figure*}
\captionsetup[subfigure]{justification=centering}
    \centering
    % \begin{subfigure}[b]{.25\textwidth}
    %  \centering
    % \includegraphics[width=.59\textwidth] 
    % {figures/experiments/varyingSALES/varyep.png}
    % \includegraphics[width=.49\textwidth] 
    % {figures/experiments/varyingSALES/varyacc.png}
    % \end{subfigure}
    \begin{subfigure}[b]{.24\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experiments/varyingSALES/varyep.png}
    \caption{Ex-Post DP $\epsilon$}
    \label{fig:varEp}
    \end{subfigure}
    \begin{subfigure}[b]{.251\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experiments/varyingSALES/varyacc.png}
    \caption{FNR and FPR}
    \label{fig:varEnt}
    \end{subfigure}
    \begin{subfigure}[b]{.24\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experiments/distrib/epDist.png}
    \caption{Ex-Post DP $\epsilon$}
    \label{fig:distEp}
    \end{subfigure}
    \begin{subfigure}[b]{.25\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experiments/distrib/fnrDist2.png}
    \caption{FNR and FPR}
    \label{fig:distEnt}
    \end{subfigure}
   %  \begin{subfigure}[b]{.285\textwidth}
    
   %  \centering
   %  \includegraphics[width=\textwidth]{figures/experiments/varyingSALES/varyacc.png}
   % \caption{FNR and FPR}
   % \label{fig:varFNRFPR}
   %  \end{subfigure}
    \caption{Privacy ($\epsilon$,$\mathcal{H}_{min}(\Theta)$) at $\gamma=0.0005$ for varying $u$ (a-b) and for two equivalent query trees (c-d) on Sales data}
    \label{fig:varyingdistrib}
\end{figure*}

==> notationtable.tex <==

\begin{table}[]
\begin{tabular}{|l|l|}
\hline
\textbf{Notation} & \textbf{Represetnation}       \\ \hline
N                 & The set of negaitves          \\ \hline
P                 & The set of positives          \\ \hline
$\beta$-FNR       & Bound for false negative rate \\ \hline
\end{tabular}
\caption{Notation Table \xh{either complete it or remove it, depending on space}}\label{tb:notation}
\end{table}

==> revisionletter.tex <==
\onecolumn
\begin{center}
    \LARGE{
    \textbf{\sc\textbf{ProBE:}  Proportioning Privacy Budget for Complex Exploratory Decision Support} }\\
    \normalsize{Revision Letter} \\
    \textcolor{gray}{CCS'24, Paper Submission \#2040}
    % \reviewer{\normalsize{VLDB'22, Paper 854}} 
\end{center}

We sincerely thank the reviewers for the insightful and constructive feedback given on our submission, as well as the opportunity to improve the paper in the aspects specified. We first summarize our overall revisions, then explicitly describe all of the revisions performed as they relate to the responses provided to each reviewer below, and highlight each change in the paper in \textcolor{blue}{blue}.
\\

\noindent
\textbf{Overall Revisions}
\\

\noindent
{\color{gray} Dear Author(s),
Please revise and improve your submission to address the following comments from reviewers:
\begin{enumerate}
    \item Improve the paper’s presentation, including:
    \begin{enumerate}
        \item Clarification of motivations for complex queries with use cases/examples/applications
        \item Clarification on the exact queries covered.
        \item Discussion of the related work on DP over join queries and show the connection/difference between the complex queries and join queries.
        \item Including ProBE-Ent in the main paper.
        \item Addressing other comments from reviewers.
    \end{enumerate}
    \item Provide a concrete theoretical analysis of the computation cost and compare it with current DP+SQL approaches.
    \item Including an additional discussion on exploring ProBE in the context of relaxations such as (epsilon, delta), Renyi, f-DP, etc.
    \item Provide an explanation of how Phase 1 and Phase 2 of the algorithm interact, specifically detailing the optimization process between these two phases, if possible.
    \item Experimental Evaluation:
    \begin{enumerate}
        \item Add results from the naive approach with the second step.
        \item Clarify the importance of the first step in the evaluation process.
        \item Provide a criterion for setting the values of accuracy requirements $\alpha$ and $\beta$ appropriately, and add additional experiments on different values of $\alpha$ and $\beta$ to justify the selection criterion.
        \item Provide additional experiments to justify whether the half-half budget allowance between two phases on $\beta$ is optimal.
    \end{enumerate}
\end{enumerate}~\\
}


We have addressed all of the comments above by providing the following revisions to our submission:

\begin{enumerate}
    \item We have improved the paper's presentation in terms of the following:
    \begin{enumerate}
        \item We have clarified the motivation for the complex queries we tackle and added use cases/examples in the Introduction section on page 1.
        \item We have added further detailed explanations on the nature of the queries that we cover in our paper by adding and modifying the query definitions in section 3.1 on page 3.
        \item We have added a discussion of previous work as it relates to join queries and have compared these queries to our complex queries by adding a clarification in the Previous Work  (section 7) on page 11, as well as the extended version of the Previous Work section in Appendix D on page 22.
        \item We have included ProBE-Ent in the main paper by adding the 5.3 subsection entitled "Multi-Step Entropy-based Algorithm" on page 10, and we have included the results of this algorithm in the Experimental Results section 6 in Figures 6, 7 and 8. We have added a brief analysis of this algorithm's performance in comparison to the other algorithms in section 6.2 on page 11. Finally, we have only included the Min-Entropy results in Appendix F (additional experiments) to avoid redundancy.
        \item We have addressed other comments from reviewers which we will detail below.
    \end{enumerate}
    \item We have provided a theoretical analysis of the computational cost of ProBE as it relates to traditional SQL queries by adding section B in the Appendix entitled "ProBE Computational Complexity Analysis" on page 20.
    \item We have included a discussion on adapting the ProBE framework to be implemented with different relaxations of DP such as (epsilon,delta) DP, Renyi DP, f-DP at the end of section 4.1 on page 6.
    \item We have provided an explanation in our response to R4.D7 that the two phases interact by optimizing the selection of the optimal uncertain region parameter $u_{opt}$ for Phase Two by using the results of Phase One and estimating an upper bound on the FPR resulting from the first phase. This upper bound is subsequently used to determine if Phase Two is necessary (by comparing it to $\alpha$), which then computes the optimal $u$ and reruns the shift algorithm to meet the bound. Due to this optimization of the $u$ parameter, we choose to fix the split of $\beta$ budget, but provide additional experiments to explore further possible splits in Appendix F (additional experiments).
    \item We have improved our experimental evaluation section as follows:
    \begin{enumerate}
        \item We have added the results of using the naive approach (i.e. splitting the $\beta$ budget equally across sub-queries) as Phase One of ProBE in the experimental section 6.2 and have entitled it ProBE-Naive. We have included this algorithm in Figures 6, 7, 8 in the main paper as well as Figures 9, 10, 11 in Appendix F (additional experiments) which replaced the "ProBE-SS" to ensure consistency with the main paper.
        \item We have further detailed the importance of Phase One in ProBE by adding a paragraph entitled "Comparison of Naive versus Optimized Phase One" in section 6.2 on page 11 which compares the results of ProBE-Naive versus ProBE to highlight the role of the optimization in Phase One.
        \item  We have clarified that the accuracy requirements $\beta$ and $\alpha$ are user-set bounds and are dependent upon the use case of the decision support application built upon ProBE in section 3.1 on page 4. We have also added experiments to explore the effect of setting different values for the $\alpha$ and $\beta$ bounds and to highlight that ProBE allows for the user/data analyst to set any desired accuracy bound with the guarantee that they will be met with minimal privacy loss. These experiments are included in Figure 8 on page 14 along with their analysis in a paragraph entitled "Varying $\beta$ and $\alpha$ Parameters" on page 12.
        \item We have provided additional experiments which explore different budget splits for the $\beta$ budget across the two phases of ProBE in Appendix F on page 23. These results show that it is non-trivial to determine the optimal $\beta$ budget split across the two phases as the difference in privacy results is negligible and not consistent in pattern. Nevertheless, the optimization of the budget distribution between the two phases is an interesting direction we are currently considering.
    \end{enumerate}
\end{enumerate}

\noindent
\textbf{Reviewer 1}
\\

\noindent
\textcolor{gray}{D1. Have you tried running the naive approach but with your second data-dependent improvement step?}

 We have added the ProBE algorithm with the Naive approach as the first step to our experiments (in Figures 6, 7, 8) and have entitled it ProBE-Naive. We have also highlighted the importance of the optimization in Phase One in the paragraph entitled "Comparison of Naive versus Optimized Phase One" in section 6.2 at the end of page 11 as follows: 
 
 "Comparison of Naive versus Optimized Phase One. By analyzing the difference in results between the  ProBE-Naive and ProBE algorithms, we are able to highlight the importance of the $\beta$ budget optimization performed by ProBE in Phase One. In cases where query sensitivities and domain sizes dramatically differ (i.e. resulting in vastly different uncertain regions) across sub-queries, the optimal distribution would be to allocate a smaller $\beta$ budget for the sub-query with the larger uncertain region $u$ as they are inversely correlated (a direct reflection of the trade-off between FN and FP), and allocate a larger $\beta$ to the sub-query with a smaller $u$. In cases such as this, the Naive approach would result in a non-optimal equal distribution of the $\beta$ budget and subsequently a higher privacy loss. We see this difference in privacy loss in Figure \ref{fig:privacyres} in specific cases such as the Sales (row 2) and UCI (row 3) datasets where the addition of specific sub-queries results in a much higher privacy loss depending on underlying the data distribution. "
 
 Finally, we have updated the additional experiments in Appendix F ( Figures 9, 10, 11) to replace ProBE-SS with ProBE-Naive to ensure consistency across the entire paper.
\\

\noindent
\textcolor{gray}{D2. Have you considered comparing the approach against an iterative one that is data-dependent for both FNR and FPR bounds?}

As for extending ProBE to be iterative and data-dependent for both FPR and FNR, our entropy-based approach in the Appendix is designed for exactly that purpose; and its performance comparison indeed shows that the iterative approach  (ProBE-Ent) improves privacy loss further. We have included ProBE-Ent in the main paper by adding a new subsection numbered 5.3 and entitled “Multi-Step Entropy-based Algorithm” on page 10. We have also included ProBE-Ent in the experimental section 6.2 in Figures 6, 7, 8 and have updated the experimental analysis to include their results as well. Specifically, we have added the following paragraph in section 6.2 on page 11: 

"The iterative, entropy-based algorithm ProBE-Ent achieves close or
the lowest privacy loss overall. This is due to the fact that ProBE-
Ent makes use of the underlying data distribution to progressively
compute the results of the query at the lowest privacy cost, while
also allowing for early stopping at a much lower privacy loss if all
predicates are properly classified outside of the uncertain region." 

We have also updated phrases such as "two algorithms" or "the ProBE algorithm" to include the additional algorithms evaluated. Finally, we have updated the first subsection of the additional experiments in Appendix F to only include the min-entropy results to eliminate redundancy. The subsection is now entitled "Min-Entropy Privacy Results" and includes the following paragraph:
"We extend our experiments to include Min-Entropy denoted $\mathcal{H}_{min}(\Theta)$ as part of our privacy metrics used to evaluate the performance of all algorithms. We use the same parameters as the main paper: we set a FNR bound of $\beta = 0.05$, a FPR bound of $\alpha= 0.1$, a maximum privacy loss of $\epsilon_{max} = 5$, a starting uncertain region of  $u_0=30\%|D|$ for ProBE and a default $u = 12\%$ for the Naive algorithm. We run each algorithm over a 100 iterations and vary the number of sub-queries from 1 to 6. "

"In terms of Min-entropy $\mathcal{H}_{min}(\Theta)$, the closer to $1$ the results are (meaning that the lower bound on uncertainty is extremely high) the better. The results in Figure 9 thus show that ProBE-Ent outperforms other algorithms and stays constant or suffers only from a small decrease as the number of sub-queries increases. This directly follows from the fact that ProBE-Ent is designed to maximize min-entropy at each iteration, regardless of the number of sub-queries. Other algorithms suffer from a decrease in min-entropy as the number of sub-queries increase, as it is inversely correlated to the ex-post DP loss $\epsilon$."
\\

\noindent
\textbf{Reviewer 2}
\\

\noindent
\textcolor{gray}{D1. The studied problem highlights the complex queries with multiple filter conditions. The importance of those queries needs to be addressed. In addition, complex queries involving joins are not considered. The conjunctions can be regarded as self-joins. Thus, the authors should compare related works for DP over join queries.} 

We have clarified the motivation for complex queries further by listing use cases/applications in the Introduction section on page 1 as follows:

"Other use cases for such complex queries include clinical decision support applications \cite{med1,med2,med3} which use complex queries to diagnose and classify diseases (e.g. the previously defined query), building management systems \cite{bmsds1,bmsds2} that ensure building code compliance by comparing aggregate statistics to policy thresholds, and supply management systems \cite{supply1,supply2} which optimize operations by analyzing statistics as they relate to existing benchmarks or user-defined criteria."

We have also discussed the difference between join queries and the queries we discuss and added previous work related to join queries in Section 7 page 11 as follows: 

"Join queries \cite{join1,join2,join3,join4} may be more applicable to such queries (specifically for conjunctions), but they do not encompass the full scope of the complex queries we tackle, nor does recent work apply a utility-first approach to their solutions."

As well as in the extended version of the Previous Work section in Appendix D page 22:

"Join queries may be more applicable to such queries, as conjunction-only queries may be written as join queries. However, such an approach complicates the queries at hand: the join operator is known for having high sensitivity resulting in low accuracy when answering such queries. Additionally, recent algorithms tackling join queries \cite{join1,join2,join3,join4} do not provide accuracy guarantees in terms of FNR or FPR, and their data-dependent nature make it difficult to successfully enforce error bounds."
\\

\noindent
\textcolor{gray}{D2. The authors can better introduce the background and problem definition. Which type of filter conditions and aggregations can be supported should be explicitly stated. In addition, the problem tries to list a set of outputs rather than some aggregations. How DP is proposed and guaranteed on such queries is also not clear, and the authors should describe it better. In addition, the proof in Appendix A.4 does not help. The authors should provide a step-by-step proof that the proposed mechanism satisfies equation (2).}


In short, filters can be any selection condition on records; any aggregate for which sensitivity can be computed is allowed (e.g, count, avg); DS queries (our focus) are group-by-aggregation queries with HAVING clauses which output the groups whose aggregates satisfy the condition specified in the having clause. We have improved the presentation of the problem definition and query definitions in section 3.1 page 3 by modifying the existing paragraph as follows:

"Specifically, an aggregate threshold query returns the set of objects in a dataset, deferred to as predicates, whose aggregate values exceed the set thresholds. We present the formal definitions as follows."

"Aggregate Threshold Query. An aggregate threshold query, denoted by $Q_{\mathsf{g(.)}>C}^{\Lambda,f}$,  consists of the following: (i) an aggregate function $\mathsf{g(.)}$, which includes any function whose sensitivity can be computed (e.g. AVG or COUNT); (ii) the set of predicates $\Lambda= \{ \lambda_1,\lambda_2,...,\lambda_k\}$ which represent the objects that the query iterates over to check for condition satisfaction (e.g. the set of diseases in the previous query example); (iii) a set of corresponding thresholds $C = \{c_1, c_2, ..., c_k\}$ for each predicate, and (iv) an optional filter $f$ which can be any selection condition on any column of the record."

We have also improved the presentation of our proof in Appendix A.4 to explicitly clarify how the proposed technique satisfies DP (viz. equation  (2)) on page 20 as follows:

"Third, the algorithm satisfies $\epsilon_{max}$-DP.
(i) Phase One of ProBE adds noise from the Laplace Distribution according to the Laplace Mechanism\cite{Dwork:2014:AFD:2693052.2693053}, i.e. with a mean of 0 and a standard deviation of $1/\epsilon_i$. This means that Phase one is $\epsilon_i$-differentially private.
     (ii) Phase Two of ProBE similarly adds noise from the Laplace Distribution according to the Laplace Mechanism with a newly computed $\epsilon_j$ privacy budget, making phase two  $\epsilon_j$-differentially private. 
     (iii) Because the two phases are executed sequentially, their composition (i.e. the overall ProBE mechanism) is $\epsilon_i + \epsilon_j$-differentially private. (iv) It follows that ProBE satisfies $\epsilon_{max}$-DP as it checks that the current privacy budget (i.e. $\epsilon_{i} + \epsilon_{j}$) does not exceed the limit of $\epsilon_{max}$. "
\\

\noindent
\textcolor{gray}{D3. The paper mentioned [17, 18] as related work, but the experimental evaluation only considers the native approach. These works should be included as baselines.
}

Note that due to changes to the citations, we now refer to [17] as \cite{Apex:2019:RQP:1007568.1007642} and [18] as \cite{mide}. Our naive approach is indeed an algorithm from  \cite{mide} suitably extended to deal with multiple conjuncts/disjuncts.  \cite{mide} itself is based on \cite{Apex:2019:RQP:1007568.1007642} and is strictly better than \cite{Apex:2019:RQP:1007568.1007642} for the problem studied since \cite{Apex:2019:RQP:1007568.1007642} offers no FN or FP bounds, while \cite{mide} offers a bound on FN.  We have clarified this in the paper in the “Algorithms” subsection of section 6.1 on page 11 by adding the following: "In other words, this baseline is an extension of \cite{mide} where the $\beta$ budget is split evenly across sub-queries. We do not evaluate our approach against the algorithm in \cite{Apex:2019:RQP:1007568.1007642}, as \cite{mide} is directly based on it with the additional focus on bounding the FNR only."
\\

% \textcolor{red}
% {\bf SHARAD: there is citation error above... you refer to them as [17] and [18] but they have shifted to [23] and [24]. Please correct!}

\noindent
\textcolor{gray}{D4. From my understanding, the native approach should be the same as the proposed method when there is only one subquery, as the difference between the two methods is the different way of distributing the privacy budget. The experimental results in Figure 6 show otherwise.
}

Irrespective of the number of sub-queries,  the naive approach is  “single-step” while ProBE is “two-step”.  For a single sub-query, the naive approach can be considered as the “first” of the “two” steps of ProBE with one difference: in ProBE, we set a large initial uncertain region u so as to maximize post-DP epsilon and bound the FP in step 2 of the algorithm. In contrast, in naive approach we set a smaller u, else, the resulting number of FPs would be very large.  If we choose a large u for naive, yes, indeed it would become the same as step 1 of ProBE in the case of single sub-query. We have clarified this in the paper in the “Parameters” subsection of section 6.1 by adding the following "we set this smaller default value due to the fact that the FPR is not bound in the Naive approach, meaning that a large $u$ would result in a very high FPR.", as well as in the “Privacy Results” subsection of section 6.2 on page 11 through the following: "Note that in the case of a single sub-query, the Naive and ProBE algorithms would yield the same privacy results provided that the second step of ProBE is not triggered."
\\

\noindent
\textcolor{gray}{D5. The legend in Figure 6 shows that there are four lines, but only three can be found on the figure.}

The discrepancies are because of overlapping lines in the figures. We have added the comment to address this in section 6.2 in the “Accuracy results” subsection on page 13 "hence the overlap of solid lines (FNR) for all algorithms" and by varying the size of the markers in the figures to discern the different lines. 
\\

\noindent
\textcolor{gray}{D6. The data points are indistinguishable with b/w printing.} 

We have improved the appearance of the data points in all of the Figures.
\\

\noindent
\textbf{Reviewer 3}
\\

\noindent
\textcolor{gray}{D1. Can your approach be lifted also to consider relaxations of differential privacy? }

Indeed, exploring ProBE in the context of relaxations such as (epsilon, delta), Renyi, f-DP etc. is really interesting. As we mention at the end of Sec. 4.1, other compositions of differential privacy such as the advanced composition theorem may be used in our optimization problem, but that would change the expression of the overall privacy budget in terms of the subqueries’ privacy budgets, hence changing the apportionment technique as well. For different definitions of DP, extending our framework would also necessitate a different baseline of expressing privacy loss in terms of the error rates before formulating the optimization problem. These are very interesting non-trivial directions that we are currently exploring. We have added a paragraph to discuss this aspect at the end of section 4.1 on page 6 as follows:

"Using relaxations of DP such as Rényi differential privacy \cite{renyi} or $\mathit{f}$-differential privacy \cite{fdp} is, however, non-trivial, as the expression of privacy loss $\epsilon$ in terms of the $\beta$ or $\alpha$ error rates used (i.e. as defined in \cite{mide}) may not necessarily hold. Thus, they require extensive analysis to formulate a baseline expression of privacy loss before solving the optimization problem."
\\

\noindent
\textbf{Reviewer 4}
\\

\noindent
\textcolor{gray}{D1. Definitions 2.2 and 2.3 appear to overlap significantly, seemingly conveying the same concept with inconsistent notation in the formulas.
}

Thank you for pointing out the inconsistent notation. We have modified the definition in Section 2 page 2 and now they are using the same format. 
\\

\noindent
\textcolor{gray}{D2. Essentially, the FNR (False Negative Rate) and FPR (False Positive Rate) reflect the deviation of the perturbed dataset from the original dataset. Given their fundamental similarity, why are both metrics discussed simultaneously? Wouldn't metrics like variance, which measure the deviation of the query results more directly, be more illustrative?}

Please note the type of queries that we are answering in this paper return a set of objects that satisfy the condition specified on the corresponding aggregate value in the HAVING clause, rather than the aggregate values themselves. 

Since DP adds noise to the aggregate value, the resulting noisy values when compared against conditions specified in the query may result in false positives (FP) and false negatives (FN),  also known as type 1 and type 2 errors in tasks such as information retrieval (IR),  classification, etc.  There is a trade-off between the two errors; for instance, in IR, returning all of the objects would result in 0 false negatives but a high amount of false positives. Likewise, returning no objects would result in 0 false positives but many false negatives. Similar
tradeoffs between FP and FN exist in the context of  classifiers.  Traditionally, in tasks such as IR and classification, we strive to maintain a balance between false positives and negatives simultaneously, and based on the task/application at hand, sometimes systems may pay more importance to one over the other.  To keep our discussion general and to allow different decision support settings to place different levels of emphasis on FP and FN, we discuss both the metrics simultaneously. An analyst, based on the nature of the application, may put different emphasis on the two metrics and may have different levels of tolerance to each. That is why we provide an option to specify different bounds for each metric.


Variance error, while natural to use when the system returns an aggregated value, are less suitable in our setting  because we are returning a set of answers; for instance, depending upon the query, even when the variance is high, the outcome of the query results (i.e., the set of objects satisfying the query condition) might not change and, thus, variance may not affect the resulting set.  Measures such as FP and FN are more suitable instead as explained above. We have added the discussion explaining our choice of the metric at the end of Section 3.1 on page 4 by including the paragraph below:

"Note that in our framework, the $\beta$ and $\alpha$ accuracy bounds are user-set parameters and depend largely on the nature of the overarching decision support application; for instance, a medical diagnosis application may choose to emphasize the FNR over the FPR if the absence of disease detection is more crucial than an erroneous detection. This model is motivated by similar models used in statistical inference which is used to control false negative and/or positive errors \cite{statinf1}. Additionally, we choose to focus on FNR/FPR over other accuracy measures due to the nature of the queries we tackle, which return a set of objects rather than aggregate values. For instance, a different metric such as variance error may yield a high error value for a specific query whereas the returned set remains unchanged, thus not precisely reflecting the accuracy of the results."
\\

\noindent
\textcolor{gray}{D3. Existing SQL queries typically support conjunction or disjunction types directly. It seems more logical to apply noise after the query result rather than performing two separate queries followed by conjunction or disjunction computation. This approach seems to add noise in two rounds unnecessarily.
}

Our queries are set-based queries where we return the entities (referred to as predicates in the paper)  which satisfy the condition set by the HAVING clause, therefore we cannot add noise after running the query because we are not returning aggregate values but rather a set of objects. Adding noise at the end is also contingent upon computing the sensitivity of the query, which may be difficult for such complex queries.
\\

\noindent
\textcolor{gray}{D4. The proposed ProBE in the paper requires multiple steps to optimize privacy loss and budget allocation, especially involving the decomposition of complex queries and reallocation of budgets. It would be better if the author could analyze the computational complexity of ProBE and compare the complexity with the existing SQL queries.}


As implied by the reviewer in their comment, query execution in ProBE, as alluded to in the paper, indeed incurs k times the computational overhead compared to the executing the query in SQL systems, if the query contains k conditions in the HAVING clause.

We, however, note that this is based on the naive implementation of PROBE which can be significantly optimized. Our focus in the paper is developing a technique to simultaneously provide utility bounds on FP and FN while answering the query in a differentially private manner maximizing privacy. We did not attempt to optimize execution overhead which we believe are interesting directions of future work. Indeed, such overheads can be brought down to be negligible with a careful implementation and some changes to the underlying database implementation. We explain this using the following query as an example.

\begin{verbatim}
SELECT disease, count(*) FROM PATIENT_DATA
WHERE disease_type ='viral'
GROUP BY disease
HAVING (count(*) > c1 AND avg(age) > 65) 
\end{verbatim}


A typical query plan to execute such a query is listed below (indeed, this plan is directly lifted from MySQL using the EXPLAIN command). 

\begin{enumerate}
    \item Full Table Scan on $PATIENT\_DATA$
    \item GROUP BY disease attribute
    \item Compute aggregations on $count(*)$ and on avg(age) based on the tuples in a group per group and filter matching groups based on the count(*) > c1 and avg(age) > 65 conditions
    \item Return matching groups
\end{enumerate}

Now, if we were to implement the query in ProBE using a naive strategy, we will answer two sub-queries Q1 (with the HAVING condition count(*) > c ) and Q2 (with the HAVING condition avg(age) > 65) which will result in the following execution plan:

For Q1:
\begin{enumerate}
    \item Full Table Scan on $PATIENT\_DATA$ 
    \item GROUP BY disease attribute
    \item Compute aggregations with noise on count(*)  based on the tuples in a group per group and filter matching groups based on count(*) > c1 condition 
\end{enumerate}

For Q2:
\begin{enumerate}
    \item Full Table Scan on $PATIENT\_DATA$ 
    \item GROUP BY disease attribute
    \item Compute aggregations with noise on avg(age)  based on the tuples in a group per group and filter matching groups based on avg(age) > 65 condition

\end{enumerate}

And lastly:
\begin{enumerate}
    \item Compute conjunction of Q1 and Q2
    \item Return matching groups
\end{enumerate}


This, as the reviewer suggests, will add complexity - in fact, if the HAVING condition has k conditions, the complexity of executing the query would be roughly k-times the complexity of executing a single query. However, such overheads can be alleviated by a slightly smarter implementation. In particular, when we scan for each of the sub-queries, we do not need to do this scan independently. A better plan would be:

\begin{enumerate}
    \item Full Table Scan on $PATIENT\_DATA$
    \item GROUP BY disease attribute
    \item Compute all aggregations with noise i.e. count(*) and avg(age) and filter matching groups based on the count(*) $>$ c1 and avg(age) $>$65 conditions 
    \item Compute conjunction of Q1 and Q2
    \item Return matching groups
\end{enumerate}

The above execution plan would meet our requirement, and has complexity similar to the original SQL plan, but will require database implementation to be slightly modified  to share the scan across sub-queries to achieve the above. 


As mentioned earlier, our goal in the paper is to develop a framework for answering queries with appropriate guarantees of utility and privacy. Details for implementation/realization of the technique in databases remains an important direction for future work. Nonetheless, to address the reviewers comment, we have added a new section in Appendix B entitled "ProBE Computational Complexity Analysis" on page 20.
\\

\noindent
\textcolor{gray}{D5. The experiments discuss the results of performing multiple rounds of conjunction or disjunction operations on simple query results. However, given that this paper's method decomposes all queries into atomic queries and perturbs each individual atomic query, there theoretically could be issues with complex query results receiving duplicated noise additions. There needs to be a more detailed discussion of the experimental results on complex queries, for example, (Q1 or Q2) and Q3 <=> (Q1 and Q3) or (Q2 and Q3). The experiments should analyze whether adding noise to atomic queries could lead to inequivalent outcomes in equivalent logical operations. If disparities exist, the reasons behind these differences and their severity should be clarified. Such propositional logic operations are widely used in discrete mathematics, and the same principles apply to complex queries.}

The disparity between rewriting a complex query in different but logically equivalent expressions has been evaluated in the “distribution” experiment (Figure \ref{fig:varyingdistrib} (c) and (d)) where we compare the performance of ProBE when running the query Q1 OR (Q2 AND Q3) versus (Q1 OR Q2) AND (Q1 OR Q3) where results show that the two queries do end up with a different privacy budget, specifically the distributed query has a higher privacy loss due to the allocation of an additional budget to Q1 as it appears twice. We have provided the following additional explanation in section 6.2 at the end of the Distribution experiment on page 12 "This is attributed to the fact that $Q_1$ was allocated an additional privacy budget due to its second occurrence in $Q_{II}$, thus incurring a higher cost on the overall privacy loss due to the use of the Sequential Composition theorem."
\\
% \color{red}{\bf SHARAD: there is a missing reference Figure x above}

\noindent
\textcolor{gray}{D6. Regarding the issue of measuring privacy loss, Equation 12 suggests that the sequence composition theory of Differential Privacy (DP) can be utilized to measure the consumed privacy budget. However, the practical concern is that the sequence composition requires the original datasets to be independently distributed, and the input datasets x1 and x2 for the queries f1(x1) and f2(x2) must not have any intersection to ensure applicability. But how to ensure this? Following the necessity proposed in this paper, which decomposes all queries into atomic queries, executing complex query mechanisms necessitates the combination of multiple atomic queries. Such an approach significantly increases the privacy consumption compared to directly conducting a query using SQL functions and then adding noise once. Consequently, the trade-off between privacy and utility becomes markedly unreasonable in this context.
}

There may be some confusion; The sequential composition theorem of DP does not require the original datasets to be independently distributed but rather the parallel composition theorem does. Thus, the input data may have intersection. 
\\

\noindent
\textcolor{gray}{D7. When implementing the ProBE, half of the $\beta$ budget is allocated to each phase. Why do you do this half-half budget allocation? Could you provide an analysis of optimizing the budget allocated to the two phases? Another concern is that the relationship between Phase 1 and Phase 2 is not clear enough; it seems that Phase 2 just uses the output from Phase 1, is there any optimization between the two phases?
}

In our paper, we primarily focus on optimizing the beta budget allocation within the phases (hence the apportionment of beta in terms of sub-queries’ beta\_i’s in each phase)  so as to minimize privacy loss rather than across phases. Between phases, we choose to optimize the uncertain region parameter u, primarily because our guarantee on the FNR bound (beta) is already met, but the FPR bound (alpha) may not be at the end of phase 1. Due to our varying of the uncertain region parameter u between phase 1 and phase 2, we chose to fix the beta parameter. The optimization of distributing beta between phases is an interesting question that we are currently considering. We have included an additional experiment (Table 3) which explores different distributions of the beta budget across the two phases in Appendix F page 22-23, and have included the analysis below:

"Varying $\beta$ budget split across phases. We evaluate the privacy loss and accuracy measures of our proposed ProBE algorithm when varying the distribution of the overall $\beta$ bound budget across the two phases of the algorithm. We use the following combinations of percentages: $\{10\%-90\%$, $90\%-10\%$, $50\%-50\%$, $40\%-60\%$, $60\%-40\%$, $\}$ where the first percentage is allocated to Phase One of ProBE and the second is allocated to Phase Two. We use a simple disjunction query $Q_1 \cup Q_2$ on the Taxi dataset with the parameters of $\beta=0.05$, $\alpha=0.1$. Our results are shown in Table \ref{tab:varbeta}. The different distributions used for the $\beta$ budget do not significantly impact the privacy loss $\epsilon$. There is no direct correlation observed between privacy loss and the $\beta$ distribution across the two phases, as we observe that although the lowest privacy loss achieved is when $90\%$ of $\beta$ is allocated to the Phase One, this is not the case for the $60\%$ allocation. We additionally note that the FPR is the highest when Phase One is allocated $90\%$ of $\beta$ and lowest when $90\%$ is allocated to Phase Two, but the FPR bound of $\alpha = 0.1$ is upheld regardless of the split."

As well as a pointer to this experiment in section 5.1 page 8 i.e. "However, we explore different $\beta$ allocation strategies across the two phases in Appendix F."
\\

\noindent
\textcolor{gray}{D8. Algorithm 3 is confusing because it combines the definition of the EstimateFPs( ) function. It would be more friendly to readers if you could put the definition in a separate table.}

We have improved the algorithm presentation by adding a new algorithm box entitled "estimateFPS" in section 5.2 page 9.
\\

\noindent
\textcolor{gray}{D9. The setting of accuracy requirements $\alpha$ and $\beta$, dependent on dataset types. However, it may increase the risk of privacy leakage if set too high or exceed the dataset's acceptable range if set too low. Is there a criterion for setting the values of accuracy requirements appropriately? More discussions on how to select the values could be provided.}

These accuracy bounds are user-set and depend largely on the nature of the decision support application; for example, a medical diagnosis application may choose to emphasize false negatives over false positives if the lack of detection of such disease is more crucial than a false detection. We have included such a discussion at the end of section 3.1 page 4. We have also included additional experiments to highlight the effect of differing values for alpha and beta in the experimental section 6.2 in Figure 8 (page 14) along with a paragraph entitled "Varying $\beta$ and $\alpha$ Parameters" (page 12) with the following analysis:

"Varying $\beta$ and $\alpha$ Parameters.
We analyze the effect of selecting different values for the user-set FNR bound $\beta$ and FPR bound $\alpha$ on all four algorithms. We vary the two bounds by setting their values to $\{0.025, 0.05, 0.075, 0.1, 0.125, 0.15\}$ on the Taxi dataset with a 3-disjunction query (i.e. $Q_1 \cup Q_2 \cup Q_3$). 
Figure \ref{fig:varyAB} (a) shows that varying $\beta$ causes privacy loss $\epsilon$ to decrease as $\beta$ increases across all algorithms, which is to be expected due to the inverse correlation between $\epsilon$ and $\beta$. The accuracy measures depicted in Figure \ref{fig:varyAB} (b), i.e. the FNR and FPR, are not significantly impacted as their respective bounds are met by the ProBE-based algorithms. 
Conversely Figure \ref{fig:varyAB} (c-d) depicts the effect of varying the $\alpha$ bound on FPR. As the Naive algorithm does not support a mechanism to bound the FPR, the privacy and accuracy results remain constant.  On the other hand, we note that the privacy loss $\epsilon$ also decreases as the $\alpha$ bound is increased for ProBE-based algorithms. 
This is attributed to the fact that, as the $\alpha$ bound increases, the probability of Phase Two being run decreases as the tolerance for FP errors is higher, thus avoiding the additional privacy cost of the second step. However, this decrease is dependent upon the data distribution and how many elements are in the uncertain region; if the estimated FPR is lower than a smaller bound (e.g. $0.1$) then increasing $\alpha$ will have no additional on privacy loss, hence the somewhat constant FPR between $0.1-0.15$ for the ProBE-based algorithms. 
In terms of accuracy, the FNR and FPR similarly do not see a significant change, as their respective bounds are met regardless of their values. Setting a value for the $\beta$ and $\alpha$ bounds are thus entirely dependent on the use case of the decision support application built upon our ProBE algorithm and its purpose, as well as the underlying data distribution. Therefore, ProBE allows the user the flexibility of exploring the trade-off between privacy and accuracy in a way that meets their various requirements."


\newpage
\setcounter{page}{1}
